Communicating with Speakers and Listeners of Different Pragmatic Levels

This paper explores the impact of variable pragmatic competence on communicative success through simulating language learning and conversing between speakers and listeners with different levels of reasoning abilities. Through studying this interaction, we hypothesize that matching levels of reasoning between communication partners would create a more beneficial environment for communicative success and language learning. Our research findings indicate that learning from more explicit, literal language is advantageous, irrespective of the learner's level of pragmatic competence. Furthermore, we find that integrating pragmatic reasoning during language learning, not just during evaluation, significantly enhances overall communication performance. This paper provides key insights into the importance of aligning reasoning levels and incorporating pragmatic reasoning in optimizing communicative interactions.

==> commenting_macros.tex <==
%% commenting macros

% use this to hide larger blocks of material:
% \renewcommand{\hide}[1]{}

\usepackage{xcolor}
\usepackage{amssymb}

%for fancier colors use the following options when defining your document class
%\documentclass[usenames,dvipsnames]{article}
%then you can define colors as follows:
%\colorlet{macolor}{WildStrawberry!100}


\definecolor{hhcolor}{rgb}{0.2,0.6,0.6}
\definecolor{pmcolor}{rgb}{0.4,0.2,0.1}
\definecolor{etncolor}{rgb}{0.4,0.5,0.1}

\definecolor{todocolor}{rgb}{0.9,0.1,0.1}
\definecolor{changedcolor}{rgb}{0.42,0.27,0.57}
\definecolor{removedcolor}{rgb}{0.867,0.176,0.361}

\newcommand{\nbc}[3]{
		{\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
		{\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}
}

\newcommand{\hh}[1]{\nbc{HH}{#1}{hhcolor}}
\newcommand{\pmangg}[1]{\nbc{PM}{#1}{pmcolor}}
\newcommand{\etn}[1]{\nbc{ETN}{#1}{etncolor}}
\newcommand{\kn}[1]{\nbc{KN}{#1}{etncolor}}
\newcommand{\fao}[1]{\nbc{FaO}{#1}{pmcolor}}

\newcommand{\todo}[1]{\nbc{TODO}{#1}{todocolor}}
\newcommand{\changed}[1]{\nbc{CHANGED}{#1}{changedcolor}}
\newcommand{\removed}[1]{\nbc{REMOVED}{#1}{removedcolor}}
\newcommand{\hhcheck}[2][1=]{\todo[linecolor=purple,backgroundcolor=purple!25,bordercolor=purple,#1]{{\bf HH, please check:} #2}}

% Use this to temporarily hide reviewing comments, todos, etc.:
% \renewcommand{\anna}[1]{}
% \renewcommand{\hh}[1]{}
% \renewcommand{\pmangg}[1]{}
% \renewcommand{\etn}[1]{}
% \renewcommand{\todo}[1]{}
% \renewcommand{\removed}[1]{}

% Use this to make "changed" items appear normal:
% \renewcommand{\changed}[1]{#1}

%% end commenting macros

==> tables/easiest_env.tex <==
\begin{tabular}{lcll}
\toprule
{} & {Listener train \& eval } & {Easy}  & {Hard} \\
\midrule
a) &  0 &    91.2 &   80 \\
b) &  2   &  93.7** &  84.5** \\
\bottomrule
\end{tabular}


==> tables/hard_env.tex <==
\begin{tabular}{lcl}
\toprule
{} & {Listener }  & {Accuracy} \\
\midrule
a) &  0  &   80.8 \\
b) &  2  &  84.7** \\
c) &  4  &   85.4** \\
\bottomrule
\end{tabular}

==> tables/listener_basic.tex <==

\begin{tabular}{lccl}
\toprule
 & \multicolumn{2}{c}{Listener} & \\
{} & Training & Evaluation & {Accuracy} \\
\midrule
a) & 0 & 0 & 85.4 \\
\hline
b) & 0 & \multirow{2}{*}{2} &  85.7 \\
c) & 2 &  &  87.6** \\
\hline
d) & 0 & \multirow{2}{*}{4} &  85.8 \\
e) & 4 &  &  88.2** \\

\bottomrule
\end{tabular}


==> tables/speakers_table.tex <==
\begin{tabular}{lccl}
\toprule
{} & {Listener } & {Speaker train} & {Accuracy} \\
\midrule
a) & \multirow{2}{*}{0} &  1 &   $80.8$** \\
b) &  &  3 &  $79.2$ \\
\hline
c) & \multirow{2}{*}{2}  & 1  &   $84.7$** \\
d) &  & 3 &   $83.4$ \\
\hline
e) & \multirow{2}{*}{4}  & 1 &  $85.4$** \\
f) & & 3 & $84.1$ \\

\bottomrule
\end{tabular}

